Integrated Control and Active Perception in POMDPs for Temporal Logic Tasks and Information Acquisition

This paper studies the synthesis of a joint control and active perception policy for a stochastic system modeled as a partially observable Markov decision process (POMDP), subject to temporal logic specifications. The POMDP actions influence both system dynamics (control) and the emission function (perception). Beyond task completion, the planner seeks to maximize information gain about certain temporal events (the secret) through coordinated perception and control. To enable active information acquisition, we introduce minimizing the Shannon conditional entropy of the secret as a planning objective, alongside maximizing the probability of satisfying the temporal logic formula within a finite horizon. Using a variant of observable operators in hidden Markov models (HMMs) and POMDPs, we establish key properties of the conditional entropy gradient with respect to policy parameters. These properties facilitate efficient policy gradient computation. We validate our approach through graph-based examples, inspired by common security applications with UAV surveillance.

==> fig/task2-dfa.tex <==

\begin{tikzpicture}[->, >=stealth, shorten >=1pt, auto, node distance=1cm, semithick]
  % Define nodes
  \node[draw, circle, fill=orange!20] (0) {$q_0$};
  \node[draw, circle, below left= of 0,fill=  blue!20] (1) {$q_1$};
  \node[draw, circle, below right=  of 0,fill=red!20] (2) {$q_2$};
    \node[draw, circle, below left= of 1,fill=blue!20] (3) {$q_3$};
    \node[draw, circle, below right=  of 1,fill=blue!20] (4) {$q_4$};
    \node[draw, circle, below left=  of 4,fill=blue!20,accepting] (5) {$q_5$};
    \node[draw, circle, below right=  of 2,fill=red!20, accepting] (6) {$q_6$};
   \path[->] (0) edge node {$\neg\tau$} (1)
   (1) edge node {$a$} (3)
    (1) edge [loop above] node {$\neg a \lor \neg b$} (1)
 (1) edge node {$ b$} (4)
  (4) edge node {$b$} (5)
(3) edge node {$a$} (5)
(0) edge node {$\tau$} (2)
(2) edge [loop above] node {$\neg p_v$} (2)
(2) edge node {$p_v$} (6);
\end{tikzpicture}


==> intro.tex <==
Probabilistic planning in \ac{mdp}s with temporal logic under imperfect information presents several fundamental challenges: In partial observation settings, the planner lacks access to the underlying state trajectory, making it uncertain about the sequence of temporal events that have occurred. This uncertainty propagates to the task progress state, making it difficult to determine whether a given temporal logic specification has been satisfied.  A classical approach is to construct a product between the underlying \ac{mdp} and an automaton expressing the temporal logic formula, and maintain a belief state over the product state space. Due to this product operations, the set of supports  of beliefs grows exponentially, making planning intractable  for complex temporal logical  formulas. % Furthermore, satisfying a temporal logic formula often results in delayed and sparse rewards, further compounding the challenges of a large belief space. %
 %   This sparsity leads to exploration failures in sampling-based \cite{silverMonteCarloPlanningLarge2010b} and point-based solvers \cite{shaniSurveyPointbasedPOMDP2013} for Partially Observable MDPs (POMDPs), making it difficult to efficiently learn optimal policies.


To address these challenges, uncertainty quantification plays a crucial role in decision-making under partial observability. Explicitly minimizing   task satisfaction uncertainty in  POMDP planning can  enable more efficient information gathering and reduce ambiguity in assessing task completion. To this end,  this paper introduces a class of POMDPs with \emph{both controllable transition and controllable observation functions}, where the task specifications are expressed in linear temporal logic over finite traces (LTLf). The model  explicitly allows actions to actively elicit information in   stochastic environments to minimize uncertainty in task satisfaction assessment. Specifically, we introduce an information-theoretic performance metric, measured by the remaining uncertainty regarding the task  completion   estimation given observations. The objective is to design a \emph{joint control and active perception policy in POMDPs} that  maximizes the probability of task completion while minimizing the uncertainty in self-assessment of task completion.

Motivated with recent progress in using natural policy gradients for MDPs/POMDPs \cite{} and the need to mitigate belief explosions, we then develop a policy gradient-based approach to compute a (local) optimal joint control and active perception policy. Building on our prior work on active perception in hidden Markov models (HMMs),  we develop a method  for computing the control and perception policy gradient of the conditional entropy in task completion state given observations. The approach leverages the input-output observable operator models \cite{thonLinksMultiplicityAutomata2015} for efficient computation of posterior estimate in task completion state.  

\paragraph{Related work}

\jf{Chongyang, you can start to include some related work on temporal logic planning in POMDPs, uncertainty quantification methods, and DNN for POMDPs}
